Improving ideal MHD equilibrium accuracy with physics-informed neural networks

We present a novel approach to compute three-dimensional Magnetohydrodynamic equilibria by parametrizing Fourier modes with artificial neural networks and compare it to equilibria computed by conventional solvers. The full nonlinear global force residual across the volume in real space is then minimized with first order optimizers. Already,we observe competitive computational cost to arrive at the same minimum residuals computed by existing codes. With increased computational cost,lower minima of the residual are achieved by the neural networks,establishing a new lower bound for the force residual. We use minimally complex neural networks,and we expect significant improvements for solving not only single equilibria with neural networks,but also for computing neural network models valid over continuous distributions of equilibria.

==> preamble_defs.tex <==
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\newlength{\heightOfX}\AtBeginDocument{\settoheight{\heightOfX}{X}}
\newlength{\fsize}\makeatletter
\setlength{\fsize}{\f@size pt}\makeatother
\newcommand{\nobreakbefore}{\relax \ifvmode \else \ifhmode \ifdim\lastskip > 0pt\relax \unskip\nobreakspace \fi \fi \fi }\let\oldcite\cite
\renewcommand{\cite}{\nobreakbefore\oldcite}\let\oldref\ref
\renewcommand{\ref}{\nobreakbefore\oldref}\newcommand{\colorboxwithoutxtraspace}[2]{\smash{\rlap{\colorbox{#1}{\phantom{#2}}}}#2}
\newcommand{\disabledprotrusion}[1]
{\ifKOMA \ifthenelseproperty{compilation}{fontspec}{\begingroup \addfontfeatures{Numbers={Lining,Monospaced}}
}{}\fi
\ifthenelseproperty{compilation}{microtype}{\microtypesetup{protrusion=false}}{}#1
\ifthenelseproperty{compilation}{microtype}{\microtypesetup{protrusion=true}}{}\ifKOMA
\ifthenelseproperty{compilation}{fontspec}{\endgroup }{}\fi
}
\makeatletter
\newcommand{\removeifnextchar}[3]
{\begingroup \ltx@LocToksA{\endgroup#2}\ltx@LocToksB{\endgroup#3}\ltx@ifnextchar{#1}{\def\next{\the\ltx@LocToksA}\afterassignment\next
\let\scratch=
}{\the\ltx@LocToksB }}
\makeatother
\newcommand*{\removeDot}{\removeifnextchar{.}{}{}}
\newcommand{\nameofperson}[1]{\textsc{#1}}
\newcommand{\Signature}[2]
{\vspace{2cm}\noindent
\begin{tabular*}{\textwidth}{@{\extracolsep{0pt}} l @{\extracolsep{\fill}} r @{\extracolsep{0pt}}}
#1,\getproperty{document}{date}	& \rule{0.33\textwidth}{1pt} 	\\
& \raggedleft{\textsc{#2}}
\end{tabular*}\vspace{1cm}}
\AtBeginDocument{\newif\ifKOMAandFancyChapterHeadings \KOMAandFancyChapterHeadingsfalse \ifKOMA \ifthenelseproperty{compilation}{fancychapterheadings}{\RedeclareSectionCommand[ beforeskip=\dimexpr3.3\baselineskip+1\parskip\relax,innerskip=0pt,afterskip=1.725\baselineskip plus .115\baselineskip minus .192\baselineskip,afterindent=false ] {chapter}\renewcommand\raggedchapter{\raggedleft}\renewcommand\chapterformat{{\fontsize{80pt}{80pt}\selectfont\textcolor{gray!25}{\thechapter}}}
\KOMAandFancyChapterHeadingstrue
}{}\fi
\ifKOMAandFancyChapterHeadings
\renewcommand\chapterlineswithprefixformat[3]{#2#3\vspace*{-.5\baselineskip}\rule{\textwidth}{.4pt}\par\nopagebreak}
\else
\fi
}
\renewcommand{\topfraction}{0.9}\renewcommand{\bottomfraction}{0.5}\setcounter{topnumber}{2}\setcounter{bottomnumber}{2}\setcounter{totalnumber}{4}\setcounter{dbltopnumber}{2}\renewcommand{\dbltopfraction}{0.9}\renewcommand{\textfraction}{0.1}\renewcommand{\floatpagefraction}{0.8}\renewcommand{\dblfloatpagefraction}{0.8}\ifKOMA
\ifthenelseproperty{compilation}{fontspec}{\DeclareTOCStyleEntry[ entryformat={ \addfontfeatures{Numbers={Lining,Monospaced}}\bfseries\sffamily\color{\getproperty{color}{main}}
},
pagenumberformat={\addfontfeatures{Numbers={Lining,Monospaced}}\bfseries\sffamily
},
]
{default}{chapter}\DeclareTOCStyleEntry[
entryformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
pagenumberformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
]
{default}{section}\DeclareTOCStyleEntry[
entryformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
pagenumberformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
]
{default}{subsection}\DeclareTOCStyleEntry[
entryformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
pagenumberformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
]
{default}{subsubsection}\DeclareTOCStyleEntry[
entryformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
pagenumberformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
]
{tocline}{figure}\DeclareTOCStyleEntry[
entryformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
pagenumberformat={\addfontfeatures{Numbers={Lining,Monospaced}}
},
]
{tocline}{table}}{}\fi
\makeatletter
\newcommand{\headlesschapter}[1]{\begingroup \let\@makechapterhead\@gobble \chapter{#1}\endgroup
}
\makeatother
\makeatletter
\newcommand\appendgraphicspath[1]{\g@addto@macro\Ginput@path{#1}}
\makeatother
\RequirePackage{xkeyval}\RequirePackage{xstring}\RequirePackage{xfp}\RequirePackage{ifthen}\RequirePackage{tikzscale}\makeatletter
\define@key{igraph}{width}{\def\igraph@width{#1}}
\define@key{igraph}{svgwidth}{\def\igraph@svgwidth{#1}}
\define@key{igraph}{angle}{\def\igraph@angle{#1}}
\define@key{igraph}{draft}{\def\igraph@draft{#1}}
\define@key{igraph}{scale}{\def\igraph@scale{#1}}
\define@key{igraph}{height}{\def\igraph@height{#1}}
\define@boolkey{igraph}{scaletext}{\def\igraph@scaletext{#1}}
\newcommand{\igraph}[2][]{\filename@parse{#2}\setkeys{igraph}{width=\linewidth}\setkeys{igraph}{svgwidth=\linewidth}\setkeys{igraph}{height=\empty}\setkeys{igraph}{scaletext=false}\setkeys{igraph}{#1}\ifthenelse{\equal{\filename@ext}{pgf}}{\typeout{----- INCLUDE pgf @ #2 ------}\let\pgfimageWithoutPath\pgfimage
\renewcommand{\pgfimage}[2][]{\typeout{----- INCLUDE pgfimgage @ ##2 ------}\pgfimageWithoutPath[##1]{\filename@area/##2}}
\resizebox{\igraph@width}{!}{\input{#2}}
}{\ifnum\pdfstrcmp{\filename@ext}{pdf_tex}=0
\typeout{----- INCLUDE pdf_tex @ #2 ------}\IfSubStr{#1}{height}{\PackageError{igraph}{pdf_tex does not allow the height attribute}{}}{}\ifthenelse{\boolean{\igraph@scaletext}}{\def\svgwidth{\igraph@svgwidth}\resizebox{\igraph@width}{!}{\import{\filename@area}{\filename@base.\filename@ext}}
}{\def\svgwidth{\igraph@width}\import{\filename@area}{\filename@base.\filename@ext}}
\else
\ifthenelse{\equal{\filename@ext}{svg}}{\typeout{----- INCLUDE svg @ #2 ------}\PackageError{igraph}{svg not implemented!}{}}{\ifthenelse{ \equal{\filename@ext}{tikz}}{\typeout{----- INCLUDE tikz @ #2 ------}\tikzsetnextfilename{\filename@base}\begin{minipage}{\igraph@width}\input{#2}\end{minipage}}{\typeout{----- INCLUDE with includegraphics @ #2 ------}\IfSubStr{#1}{height}{\includegraphics[#1]{#2}}{\includegraphics[width=\igraph@width,#1]{#2}}
}
}
\fi
}
}
\makeatother
\newlength{\imageh}\newlength{\imaged}\newlength{\imagew}\newcommand{\setimageh}[1]{\settoheight{\imageh}{\usebox{#1}}
}
\newcommand{\setimagew}[1]{\settowidth{\imagew}{\usebox{#1}}
}
\newcommand{\setimaged}[1]{\settodepth{\imaged}{\usebox{#1}}
}
\newsavebox{\imagesavebox}\newcommand{\setimagedimensions}[1]{\savebox{\imagesavebox}{\igraph{#1}}
\setimageh{\imagesavebox}\setimagew{\imagesavebox}\setimaged{\imagesavebox}}
\makeatletter
\newcommand*{\storedata}[2]{\count@=0 \@tfor\@tmp:=#2\do{ \advance\count@\@ne \expandafter\let\csname data:\the\count@:#1\endcsname\@tmp }\expandafter\edef\csname data:0:#1\endcsname{\the\count@}}
\newcommand*{\getdata}[2]{\@ifundefined{data:0:#2}{\@latex@error{Undefined data `#2'}\@ehc
}{\expandafter\@getdata\expandafter{ \the\numexpr \ifnum\numexpr(#1)<\z@ \@nameuse{data:0:#2}+1+
\fi
(#1)
\relax
}{#2}{#1}}
}
\newcommand*{\@getdata}[3]{\ifnum#1<\z@ \@getdata@error{\the\numexpr(#3)\relax}{#2}\else
\ifnum#1>\@nameuse{data:0:#2}\@getdata@error{#1}{#2}\else
\@nameuse{data:#1:#2}\fi
\fi
}
\newcommand*{\@getdata@error}[2]{\@latex@error{ Wrong data selector #1 for `#2',\MessageBreak which only contains \@nameuse{data:0:#2} item(s)
}\@ehc
}
\makeatother
\storedata{mydata}{{one}{two}{three}}
\storedata{mylongdata}{{one} {two} {three} {four} {five} {six} {seven} {eight} {nine} {ten}{eleven} {twelve} {thirteen} {fourteen} {fifteen} {sixteen}{seventeen} {eighteen} {nineteen} {twenty} {twenty-one} {twenty-two}{twenty-three} {twenty-four}}
\makeatletter
\RequirePackage{forarray}\RequirePackage{calc}\RequirePackage{listings}\newlength\figratiosum
\newlength\figratio
\newlength\figheight
\newlength\figwidth
\newcounter{npaths}\newcommand{\multigraph}{\begingroup \catcode`_=12 \domultigraph}\newcommand{\catcodeigraph}{\begingroup \catcode`_=11 \igraph}\define@key{multigraph}{width}{\def\multigraph@width{#1}}
\define@key{multigraph}{labels}{\def\multigraph@labels{#1}}
\newcommand{\domultigraph}[3][]{\setkeys{multigraph}{width=\linewidth - 1em}\setkeys{multigraph}{labels=\empty}\setkeys{multigraph}{#1}\setcounter{npaths}{0}\ForEachX{;}{\stepcounter{npaths}}{#2}\IfSubStr{#1}{labels}{\def\subfigurelabels{}\ForEachX{;}{\edef\subfigurelabels{\subfigurelabels"\thislevelitem"}\ifnum\thislevelcount=\value{npaths}\else
\edef\subfigurelabels{\subfigurelabels,}\fi
}{\multigraph@labels}}{}\def\paths{}\setlength\figratiosum{0pt}\def\figratios{}\ForEachX{;}{\edef\paths{\paths"\thislevelitem"}\ifnum\thislevelcount=\value{npaths}\else
\edef\paths{\paths,}\fi
\setimagedimensions{\thislevelitem}\setlength\figratio{1pt*\ratio{\imagew}{\imageh}}
\addtolength{\figratiosum}{\figratio}\edef\figratios{\figratios"\the\figratio"}\ifnum\thislevelcount=\value{npaths}\else
\edef\figratios{\figratios,}\fi
}{#2}\storedata{subcaptions}{#3}\setlength{\figheight}{1pt*\ratio{\multigraph@width}{\figratiosum}}
\addtocounter{npaths}{-1}\foreach \i in {0,...,\value{npaths}}{\pgfmathparse{{\figratios}[\i]}
\setlength\figwidth{\figheight}\pgfmathparse{\figwidth * \pgfmathresult}\setlength{\figwidth}{\pgfmathresult pt}\begin{subfigure}{\figwidth}\centering
\pgfmathparse{{\paths}[\i]}
\typeout{----- Width for multigraph figure \pgfmathresult : \the\figwidth ------}\catcodeigraph{\pgfmathresult}\endgroup
\subcaption{\getdata{\i+1}{subcaptions}}
\IfSubStr{#1}{labels}{\pgfmathparse{{\subfigurelabels}[\i]}
\label{\pgfmathresult}}{}\end{subfigure}}
\endgroup
}
\makeatother
\newcommand{\makeup}[1]{\ensuremath{ \ifluatex \symup{#1}\else
\mathrm{#1}\fi
}
}
\newcommand{\makebf}[1]{\ensuremath{ \ifluatex \symbf{#1}\else
\mathbf{#1}\fi
}
}
\input{preamble_subjects_text.tex}

==> preamble_subjects_text.tex <==
\newcommand{\vs}{vs.\xspace}
\newcommand{\eg}{e.\,g.\xspace}
\newcommand{\cf}{cf.\xspace}
\newcommand{\ie}{i.\,e.\xspace}
\newcommand{\viz}{viz.\xspace}
\newcommand{\sic}{sic\xspace}
\newcommand{\aka}{a.\,k.\,a.\xspace}
\newcommand{\wrt}{w.\,r.\,t.\xspace}
\newcommand{\etc}{etc.\xspace}

